Small surfaces of Willmore type in Riemannian manifolds

In this paper we investigate the properties of small surfaces of Willmore type in Riemannian manifolds. By \emph{small} surfaces we mean topological spheres contained in a geodesic ball of small enough radius. In particular, we show that if there exist such surfaces with positive mean curvature in the geodesic ball $B_r(p)$ for arbitrarily small radius $r$ around a point $p$ in the Riemannian manifold, then the scalar curvature must have a critical point at $p$. As a byproduct of our estimates we obtain a strengthened version of the non-existence result of Mondino \cite{Mondino:2008} that implies the non-existence of certain critical points of the Willmore functional in regions where the scalar curvature is non-zero.

==> draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}
\newcommand{\thmfamily}{}
\newcommand{\sectitlefnt}{}
\newcommand{\subsectitlefnt}{}
\newcommand{\ps@footnumber}{}

\newcommand{\authname}[1]{#1}
\newcommand{\authaddress}[1]{#1}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=136mm,totalheight=213mm,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}

  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }

  \renewcommand{\authname}[1]{\titlefamily #1\hspace*{0pt}\\}
  \renewcommand{\authaddress}[1]{\begin{minipage}{.8\linewidth}\centering\titlefamily\footnotesize
      #1\hspace*{0pt}\end{minipage}\\[1ex]}
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

